OpenMU: Your Swiss Army Knife for Music Understanding

We present OpenMU-Bench, a large-scale benchmark suite for addressing the data scarcity issue in training multimodal language models to understand music. To construct OpenMU-Bench, we leveraged existing datasets and bootstrapped new annotations. OpenMU-Bench also broadens the scope of music understanding by including lyrics understanding and music tool usage. Using OpenMU-Bench, we trained our music understanding model, OpenMU, with extensive ablations, demonstrating that OpenMU outperforms baseline models such as MU-Llama. Both OpenMU and OpenMU-Bench are open-sourced to facilitate future research in music understanding and to enhance creative music production efficiency.

==> lyricstable.tex <==
\begin{table}[t]
\centering
\scriptsize
\rastrech{1.3}
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
                                  & BLEU-1         & BLEU          & Rouge1         & RougeL         & BertScore      & Meteor         \\ \hline
\multicolumn{1}{|c|}{BART-Fusion} & \textbf{25.79} & \textbf{6.48} & \textbf{32.18} & \textbf{17.99} & 83.03          & \textbf{27.97} \\ \hline
\multicolumn{1}{|c|}{OpenMU}      & 25.60          & 5.19          & 31.31          & 17.03          & \textbf{83.14} & 27.01          \\ \hline
\end{tabular}
\end{table}

